Solving Simultaneous Target Assignment and Path Planning Efficiently with Time-Independent Execution

Real-time planning for a combined problem of target assignment and path planning for multiple agents, also known as the unlabeled version of Multi-Agent Path Finding (MAPF), is crucial for high-level coordination in multi-agent systems, e.g., pattern formation by robot swarms. This paper studies two aspects of unlabeled-MAPF: (1) offline scenario: solving large instances by centralized approaches with small computation time, and (2) online scenario: executing unlabeled-MAPF despite timing uncertainties of real robots. For this purpose, we propose TSWAP, a novel sub-optimal complete algorithm, which takes an arbitrary initial target assignment then repeats one-timestep path planning with target swapping. TSWAP can adapt to both offline and online scenarios. We empirically demonstrate that Offline TSWAP is highly scalable; providing near-optimal solutions while reducing runtime by orders of magnitude compared to existing approaches. In addition, we present the benefits of Online TSWAP, such as delay tolerance, through real-robot demos.

==> fig/delay.tex <==
{
  \begin{figure}[t!]
    \centering
    \begin{tabular}{cc}
      \begin{minipage}{0.5\hsize}
        \centering
        \includegraphics[width=0.9\hsize]{fig/raw/delay.pdf}
      \end{minipage}
      \begin{minipage}{0.45\hsize}
        \centering
        \includegraphics[width=0.9\hsize]{fig/raw/toio-with-delay.pdf}
      \end{minipage}
    \end{tabular}
    \vspace{-0.1cm}
    \caption{
      \textbf{Demo of delay tolerance.}
      \emph{left:} The initial configuration and the offline plan (accompanied by temporal orders) used in MCPs are illustrated.
      Targets are shown by the tips of arrows.
      \emph{right:} The average makespan and sum-of-costs in two scenarios are shown by ``X.''
      We made the red one's speed half in one scenario (with delay).
    }
  \label{fig:delay}
  \end{figure}
}

==> fig/instances.tex <==
{
  \begin{figure}
    \centering
    \includegraphics[width=0.5\hsize]{fig/raw/tmp.jpg}
    \caption{Instances for real robot experiment.}
    \label{fig:instances}
  \end{figure}
}


==> fig/result-eight.tex <==
{
  \begin{figure}[t!]
    \centering
    \begin{tabular}{cc}
      \begin{minipage}{0.5\hsize}
        \centering
        \includegraphics[width=0.9\hsize]{fig/raw/diagonal.pdf}
      \end{minipage}
      \begin{minipage}{0.45\hsize}
        \centering
        \includegraphics[width=0.9\hsize]{fig/raw/toio-diagonal.pdf}
      \end{minipage}
      \\
      \begin{minipage}{0.5\hsize}
        \centering
        \includegraphics[width=0.9\hsize]{fig/raw/bottleneck.pdf}
      \end{minipage}
      \begin{minipage}{0.45\hsize}
        \centering
        \includegraphics[width=0.9\hsize]{fig/raw/toio-bottleneck.pdf}
      \end{minipage}
    \end{tabular}
    \vspace{-0.2cm}
    \caption{
      \textbf{Demo with eight robots execution.}
      \emph{left:}
      The initial configurations and virtual grids are shown.
      Targets are marked by white-filled circles.
      \emph{right:}
      The results for makespan and sum-of-costs in two scenarios.
      Scatter plots of 10 repetitions are shown with transparent points.
      The points ``X'' are average scores.
      ``MCPs/F'' represents MCPs with an offline plan obtained by the makespan optimal algorithm.
      ``MCPs/E'' represents those with ECBS-TA.
    }
  \label{fig:result-eight}
\end{figure}
}
